Routing Is Not Enough: Diagnosing Intra-Adapter Subspace Contention in MoE+LoRA Fine-Tuning

Multi-domain fine-tuning often combines MoE routing with LoRA, assuming that token-level routing separates domain-specific updates. We test this assumption in MoE+LoRA using Python code paired with biomedical text and mathematical reasoning. Although these domains show near-disjoint expert routing, adding biomedical data substantially increases code perplexity, indicating that routing separation alone may not prevent negative transfer. To localize the failure, we introduce Jaccard routing overlap and adapter-gradient cosine similarity, which measure expert sharing and update compatibility, respectively. These diagnostics indicate that interference arises mostly from nearly orthogonal domain gradients competing within the same low-rank adapter subspace. We address this issue with SpawnLoRA, which dynamically adds gated sub-adapters inside MoE experts when adapter-level contention is detected, while keeping the router fixed. We evaluate SpawnLoRA on Phi-tiny-MoE-instruct and OLMoE-1B-7B across multiple mixture settings and find that it effectively reduces negative transfer compared with standard and rank-adaptive LoRA. These results demonstrate that structural separation inside experts provides benefits beyond routing or rank expansion alone.

==> experiment.tex <==
\section{Diagnosing the Failure}
\label{sec:diag}

We diagnose the source of interference in two stages. We first test the
most direct explanation: whether negative transfer is caused by the router
sending code and biomedical tokens through the same experts. After ruling
out routing overlap as the primary cause, we then examine the adapter
updates themselves and identify the mechanism of failure in gradient
space.

\paragraph{Jaccard routing analysis.}
For layer $\ell$ and training step $t$, let $S_c^{(\ell,t)}$ and
$S_m^{(\ell,t)}$ denote the sets of experts activated by code and
biomedical tokens. We measure their routing overlap using the Jaccard
score
\begin{equation}
  J^{(\ell,t)} =
  \frac{|S_c^{(\ell,t)} \cap S_m^{(\ell,t)}|}
       {|S_c^{(\ell,t)} \cup S_m^{(\ell,t)}|}.
\end{equation}
A value of 0 indicates disjoint routing paths, while a value of 1
indicates identical expert usage. On Phi-tiny-MoE, the average overlap
across layers and training steps is $\bar{J} \approx 0.056$, which
corresponds to roughly one shared expert per layer out of 64. Thus, the
router largely separates the two domains. This low overlap rules out
routing failure as the primary explanation for the observed degradation
and motivates a second diagnostic at the adapter-update level.
\paragraph{Gradient cosine similarity.}
We next measure whether the two domains produce compatible updates inside
the shared LoRA adapter. Let $g_c$ and $g_m$ be the per-domain adapter
gradients. We measure their alignment using the cosine similarity
\begin{equation}
  \cos(g_c, g_m) = \frac{g_c \cdot g_m}{\|g_c\|\,\|g_m\|}.
\end{equation}
A value of $+1$ indicates perfectly aligned updates, $-1$ indicates
directly opposed updates, and $0$ indicates orthogonal (unrelated)
updates. Across 20 trials, we find
$\cos(g_c, g_m) = -0.002 \pm 0.003$, with 75\% of measurements below
zero. The gradients are therefore not strongly opposed, but nearly
orthogonal. The shared adapter must absorb two largely unrelated update
directions within the same low-rank space.

\paragraph{Implication.}
The diagnostic narrative is therefore sequential: the Jaccard result shows
that routing overlap is too small to explain the failure, while the cosine
result identifies the actual mechanism. Even when the router sends most
tokens along different expert paths, the LoRA adapters attached to those
experts impose a shared low-rank update space. The near-zero cosine
similarity shows that code and biomedical data place nearly orthogonal
update pressures on that space. We refer to this failure mode as
\emph{intra-adapter subspace contention}. This gradient-space evidence
also indicates that the perplexity increase observed in
Section~\ref{sec:setup} is not merely a consequence of reduced code
exposure, but reflects genuine cross-domain interference. A direct
prediction follows: if the problem is contention within a shared low-rank
subspace, then simply increasing the rank of that same shared adapter may
not resolve severe conflict. Instead, capacity expansion may leave the two
domains competing within a larger but still shared adaptation space.

==> hrlora.tex <==
\section{SpawnLoRA}
\label{sec:spawnlora}

The diagnosis in Section~\ref{sec:diag} suggests a structural response to
adapter level conflict. Rather than increasing the rank of a shared
adapter, SpawnLoRA creates separate adaptation pathways inside individual
MoE experts when conflict is detected, while leaving the router unchanged.

\paragraph{Architecture.}
Each expert $E_k$ starts with a base LoRA adapter $L_{k,0}$ of rank
$r=16$. During training, the expert may additionally acquire one or more
gated sub-adapters $L_{k,1}, L_{k,2}, \dots, L_{k,J_k}$, each providing a
separate adaptation pathway. The expert output is then
\begin{equation}
  E_k(x) = W_k x + L_{k,0}(x) +
  \sum_{j=1}^{J_k} \mathrm{ReLU}(w_{k,j}^\top x) \cdot L_{k,j}(x),
\end{equation}
where $W_k x$ is the frozen pretrained expert transformation,
$L_{k,0}(x)$ is the always-active base adapter, and each sub-adapter
$L_{k,j}(x)$ is modulated by a learned gate $\mathrm{ReLU}(w_{k,j}^\top
x)$ that activates softly as a function of the input. This gives the
expert input-dependent specialisation without changing the routing
mechanism.

\paragraph{Spawn trigger.}
SpawnLoRA allocates a new sub-adapter when two signals persist within a
rolling window of training steps. First, the per-component importance
score of the existing adapter improves by less than a small threshold,
indicating that the current adapter has stopped making progress. Second,
the exponentially smoothed gap between per-domain losses exceeds a fixed
margin, indicating that the stalled progress is accompanied by an
imbalance across domains. Requiring both signals avoids spawning on
ordinary rank saturation or transient loss gaps. We additionally enforce
a minimum number of steps between allocations and cap the total
sub-adapters per expert. Exact hyperparameter values are listed in
Appendix~\ref{app:hyperparams}.

\paragraph{Initialisation.}
At allocation, the new sub-adapter is initialised so that its output
direction matches the part of the gradient signal that the existing
adapter has failed to capture. Concretely, the $A_{k,j}$ matrix is set
from the top $r$ left singular vectors of the \emph{residual gradient}
$\nabla_W \mathcal{L}$, that is, the component of the loss gradient that
lies outside the subspace already spanned by the base adapter. The
$B_{k,j}$ matrix is initialised to zero, so the new sub-adapter
contributes nothing at the moment it is added and training remains
stable. The gate weights $w_{k,j}$ are initialised to small random
values, so the gate starts near zero and learns when to activate the new
pathway. Because sub-adapters modify only the expert's output and not
its routing inputs, adding a sub-adapter never changes which tokens are
sent to which expert.

==> methodology.tex <==
\section{Setup}
\label{sec:setup}
\paragraph{Models and domains.} 
Experiments were first conducted using Phi-tiny-MoE-instruct (1.1B active, 3.8B total parameters, 16 experts per layer with top-2 routing) and then replicated on OLMoE-1B-7B (1B active, 7B total parameters, 64 experts per layer with top-8 routing). The base weights were frozen throughout. The domain pair chosen was Python code from HumanEval \citep{chen2021evaluating} and biomedical text from PubMedQA \citep{jin2019pubmedqa}. These were intentionally selected for maximal linguistic dissimilarity, as this produces a strong and consistent interference signal that models the challenging multi-task learning scenario of high gradient conflict between disparate domains. We note the lack of more domains as a limitation (Section~\ref{sec:limitations}).

\paragraph{Conflict-scaling grid.}
We use three mixture settings with the same total of 1,550 training examples. %A very high sample count is not required to observe conflict, as the domain data ratio is the main reason of interference \textcolor{black} {(Tahmid: You need to justify this claim with proper evidence, do you have any papers to cite?)--reframed now added one extra line in the implication part to be more safe}.Since every run uses the same number of training examples, the three runs differ only in their mixture ratio.Any change across runs is therefore driven by the mixture ratio under a fixed compute and data budget, which reflects the realistic setting where a constrained budget must be allocated across domains.
Since every run uses the same total, the three runs differ only in their mixture ratio, so any change across runs is driven by mixture ratio under a fixed compute and data budget. Run A uses code only and serves as the single-domain reference. Run B uses an 80/20 code/biomedical mixture, and Run C uses a 50/50 mixture. In all settings, examples are proportionally interleaved across 1,500 training steps. We define negative transfer as the increase in held-out code perplexity relative to Run A:
\[
\mathrm{NegTransfer}
=
\mathrm{PPL}_{\mathrm{code}}(\mathrm{Run\ X})
-
\mathrm{PPL}_{\mathrm{code}}(\mathrm{Run\ A}).
\]
Because reducing the code share also reduces in-domain code exposure, this quantity jointly reflects reduced exposure and cross-domain interference; Section 4 separates these two causes through direct gradient-space diagnostics.
% \paragraph{Training.} 
% All methods were trained for 1,500 steps using the AdamW optimizer, with a learning rate set at $2 \times 10^{-5}$, a batch size of 1, and a sequence length of 512. The primary results reported are based on a single seed, however, multi-layer ablations were performed using three seeds.

% \paragraph{Baselines.} 
% The LoRA baseline \citep{hu2022lora} was configured with a fixed rank of $r = 16$. The DR-LoRA \citep{liu2024drlora} method begins at a rank of $r = 16$, incorporates six rank-expansion events, and has its router unfrozen at step 150. HRLoRA (\S\ref{sec:HRLoRA}) uses a divergence threshold of $\delta = 1.0$ nats, an importance plateau of $\tau = 10^{-4}$, and a maximum cap of $J_{\max} = 10$.

\paragraph{Baselines.} 
We compare SpawnLoRA (\S\ref{sec:spawnlora}) against a standard LoRA baseline \citep{hu2022lora} and the rank-adaptive DR-LoRA \citep{liu2024drlora} method. The primary results reported are based on a single seed although multi-layer ablations were performed using three seeds. Full hyperparameter configurations and training details for all methods are provided in Appendix B.

==> results.tex <==

\section{Confirming the Prediction}
\begin{table}[t]
\centering
\small
\begin{tabular}{llccc}
\toprule
Method & Run & Mix & PPL$_\mathrm{code}$ & NegTransfer \\
\midrule
LoRA      & A & 0\%  & 430.60  & --- \\
DR-LoRA   & A & 0\%  & 461.10  & --- \\
SpawnLoRA    & A & 0\%  & 464.92  & --- \\
\midrule
LoRA      & B & 20\% & 747.85  & $+317.25$ \\
DR-LoRA   & B & 20\% & 723.61  & $+262.51$ \\
SpawnLoRA    & B & 20\% & \textbf{684.52}  & $\mathbf{+219.60}$ \\
\midrule
LoRA      & C & 50\% & 1209.38 & $+778.78$ \\
DR-LoRA   & C & 50\% & 1773.03 & $+1311.93$ \\
SpawnLoRA    & C & 50\% & \textbf{1039.72} & $\mathbf{+574.79}$ \\
\bottomrule
\end{tabular}
\caption{Code perplexity and negative transfer on Phi-tiny-MoE-instruct.
Lower values are better for both metrics. Bold indicates the best result
within each conflict setting.}
\label{tab:main}
\end{table}

Table~\ref{tab:main} reports the main comparison on Phi-tiny-MoE-instruct.
The three methods have similar single-domain performance in Run A, with
code perplexity between 430 and 465. This makes Runs B and C more
informative, since differences in those settings mainly reflect how each
method responds to multi-domain conflict rather than large differences in
single-domain starting performance.

Under moderate conflict, SpawnLoRA achieves the lowest code perplexity and
the smallest negative transfer. The difference becomes more pronounced
under severe conflict. In Run C, DR-LoRA reaches a negative transfer of
$+1{,}311.93$, which is substantially worse than fixed-rank LoRA at
$+778.78$. Training trajectories show that DR-LoRA undergoes a perplexity
spike above 7,500 between steps 800 and 1,000 and only partially recovers
afterward. This behaviour is consistent with the diagnosis in
Section~\ref{sec:diag}. When domain gradients are nearly orthogonal inside
a shared adapter, increasing shared rank alone may not remove the source
of interference. Instead, it can leave the two domains competing within a
larger shared adaptation space.

The severe-conflict results match the qualitative prediction made by the
diagnosis. Rank expansion performs worst, fixed-rank LoRA is more stable
but still suffers substantial negative transfer, and structural separation
through SpawnLoRA performs best.


